Deformable MRI Sequence Registration for AI-based Prostate Cancer Diagnosis

The PI-CAI (Prostate Imaging: Cancer AI) challenge led to expert-level diagnostic algorithms for clinically significant prostate cancer detection. The algorithms receive biparametric MRI scans as input, which consist of T2-weighted and diffusion-weighted scans. These scans can be misaligned due to multiple factors in the scanning process. Image registration can alleviate this issue by predicting the deformation between the sequences. We investigate the effect of image registration on the diagnostic performance of AI-based prostate cancer diagnosis. First, the image registration algorithm, developed in MeVisLab, is analyzed using a dataset with paired lesion annotations. Second, the effect on diagnosis is evaluated by comparing case-level cancer diagnosis performance between using the original dataset, rigidly aligned diffusion-weighted scans, or deformably aligned diffusion-weighted scans. Rigid registration showed no improvement. Deformable registration demonstrated a substantial improvement in lesion overlap (+10% median Dice score) and a positive yet non-significant improvement in diagnostic performance (+0.3% AUROC, p=0.18). Our investigation shows that a substantial improvement in lesion alignment does not directly lead to a significant improvement in diagnostic performance. Qualitative analysis indicated that jointly developing image registration methods and diagnostic AI algorithms could enhance diagnostic accuracy and patient outcomes.

==> files/SAP-contents.tex <==
\section{Statistical Analysis Plan}
The PI-CAI (Prostate Imaging: Cancer AI) challenge led to expert-level diagnostic algorithms for clinically significant prostate cancer detection. The algorithms receive biparametric MRI scans as input, which consist of T2-weighted and diffusion-weighted scans. These scans can be misaligned due to multiple factors in the scanning process. Image
registration can alleviate this issue by predicting the deformation between the sequences. We investigate the effect of image registration on the diagnostic performance of AI-based prostate cancer diagnosis. Two registration methods are considered; rigid registration and deformable registration. The csPCa detection performance on the external testing dataset is statistically evaluated as explained in this statistical analysis plan. The study objectives are described in a predefined hierarchical tree and the tests are performed accordingly (see Figure~\ref{fig:statistical-tree}). Multiplicity is corrected for at each stage using the Holm-Bonferroni method, considering a base alpha value of 0.05. The hierarchical structure is formed following the research question as proposed in this study. Our aim is to investigate if image registration can boost model performance, in family 1A and 1B we test whether either rigid or deformable registration is better than using no registration. If one or both of these registration methods turn out to boost the performance of the AI model then we move on to testing whether model performance is better using deformable registration relative to rigid registration (family 2A) and/or whether model performance is better using rigid registration relative to deformable registration (family 2B). 

\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{figures/SAPtree.png}
    \caption{Flowchart illustrating the statistical plan to test the study objectives. The significance thresholds used for family 1A and 1B are adjusted using the Holm-Benferroni method, considering a base alpha of 0.05. If the null hypothesis of family 1A is rejected, but that of family 1B is not rejected, then we move on to testing family 2A with an alpha value of 0.05 but do not test family 2B. Conversely, if the null hypothesis for family 1B is rejected but that of family 1A is not rejected, then we move on to testing family 2B with an alpha value of 0.05, but do not test family 2A. If the null hypothesis for both family 1A and 1B are rejected, then we move on to testing both family 2A and 2B, where the significance threshold is once again adjusted using the Holm-Benferroni method considering a base alpha value of 0.05. If neither family 1A nor 1B are rejected, neither family 2A nor 2B will be tested.}
    \label{fig:statistical-tree}
\end{figure}

\paragraph{Calculation of p-values - DeLong's test}
The p-value for a superiority test comparing AUROC scores can be calculated using DeLong's test \cite{delong1988}. To test the null hypotheses as described in Figure ~\ref{fig:statistical-tree}, we use the DeLong's formulas to estimate the variance of and the covariance between the AUROC scores. In our experiments we use the faster implementation of the DeLong's algorithm, as proposed by \cite{Sun2014}. We can calculate the $z$ score using the following formula:

\begin{equation}
    z = \frac{\hat{\theta}^{(1)} - \hat{\theta}^{(2)}}{{\sqrt {\mathbb{V}[{\hat{\theta }^{(1)}}] + \mathbb{V}[{\hat{\theta }^{(2)}}] - 2\mathbb{C}[{\hat{\theta }^{(1)}},{\hat{\theta }^{(2)}}]}}}
\end{equation}

The P value is then calculated from the $z$ score using a one-tailed test. 


\bibliographystyle{splncs04}
\bibliography{bibliography}
